Two Heads Are Better than One: Model-Weight and Latent-Space Analysis for Federated Learning on Non-iid Data against Poisoning Attacks

Federated Learning is a popular paradigm that enables remote clients to jointly train a global model without sharing their raw data. However, FL has been shown to be vulnerable towards model poisoning attacks due to its distributed nature. Particularly, attackers acting as participants can upload arbitrary model updates that effectively compromise the global model of FL. While extensive research has been focusing on fighting against these attacks, we find that most of them assume data at remote clients are under iid while in practice they are inevitably non-iid. Our benchmark evaluations reveal that existing defenses generally fail to live up to their reputation when applied to various non-iid scenarios. In this paper, we propose a novel approach, GeminiGuard, that aims to address such a significant gap. We design GeminiGuard to be lightweight, versatile, and unsupervised so that it aligns well with the practical requirements of deploying such defenses. The key challenge from non-iids is that they make benign model updates look more similar to malicious ones. GeminiGuard is mainly built on two fundamental observations: (1) existing defenses based on either model-weight analysis or latent-space analysis face limitations in covering different MPAs and non-iid scenarios, and (2) model-weight and latent-space analysis are sufficiently different yet potentially complementary methods as MPA defenses. We hence incorporate a novel model-weight analysis component as well as a custom latent-space analysis component in GeminiGuard, aiming to further enhance its defense performance. We conduct extensive experiments to evaluate our defense across various settings, demonstrating its effectiveness in countering multiple types of untargeted and targeted MPAs, including adaptive ones. Our comprehensive evaluations show that GeminiGuard consistently outperforms SOTA defenses under various settings.

==> 5-discussion.tex <==
\section{Discussions}
\label{sec:discussion}
% Asides from that there are less popular \NIID types \FB has not been applied to, we further discuss two directions for improving \FB.%\xlnote{Could be moved to the appendix.}
% \subsection{Unsupervised and/or Semi-supervised Models}
% Given that currently \FB requires a labelled set for training, therefore it is of practical use to look into converting \FB into an unsupervised or semi-supervised method. One potential approach is to employ unsupervised contrastive learning~\cite{chen2020simple,radford2021learning} to train a self-supervised model that identifies malicious model updates through anomaly detection. While some research has explored this direction~\cite{yang2021cade,fergusonefficient,bansal2023cleanclip}, their applicability on \NIIDs in FL remains unknown and difficult to predict as well. On the contrary, we consider model distillation~\cite{gou2021knowledge} may be a promising technique for this purpose. Recent studies~\cite{zhu2023adfl,zhang2024badcleaner} have used model distillation to create robust student models that inherit the defense capabilities of the corresponding teacher model against backdoor attacks. We plan to look into this direction.


% \subsection{Buffer Layer}
% % We expect that better representation learning is beneficial for obtaining a more viable buffer layer for \FB. A potential direction is considering multiple layers of the model not only the PLRs.
% We view the design of buffer layer as another key direction for improving \FB. One possibility is to use enhanced representation learning to improve the effectiveness of the buffer layer in \FB. For instance, existing work~\cite{CrowdGuard,MESAS,wang2019neural,wang2019neural} found that representation learning from multiple layers rather than PLRs only can strengthen defenses against backdoor attacks. The idea is straightforward; multi-layer approaches are to capture different levels of features, from simple patterns in lower layers to complex abstractions in higher layers, therefore providing more comprehensive extraction. We plan to look into this direction as well. %Previous studies, such as those by Wang et al.~\cite{wang2019neural} and Gao et al.~\cite{gao2019strip}, have demonstrated the effectiveness of multi-layer representations in detecting and mitigating backdoor attacks.
Asides from that there are less popular \NIID types \FB has not been applied to, we believe that \FB can be further improved in the following two direction. The first direction is to convert \FB into an unsupervised or semi-supervised method. One potential approach is to employ unsupervised contrastive learning~\cite{chen2020simple,radford2021learning,yang2021cade,fergusonefficient,bansal2023cleanclip} to train a self-supervised model that identifies malicious model updates through anomaly detection. The other direction is to further improve the design of buffer layer. One possibility is to use enhanced representation learning to improve the effectiveness of the buffer layer in \FB. For instance, existing work~\cite{CrowdGuard,MESAS,wang2019neural,wang2019neural} found that representation learning from multiple layers rather than PLRs only can strengthen defenses against backdoor attacks. We plan to look into this direction as well.%While some research has explored this direction~\cite{yang2021cade,fergusonefficient,bansal2023cleanclip}, their applicability on \NIIDs in FL remains unknown and difficult to predict as well. On the contrary, we consider model distillation~\cite{gou2021knowledge} may be a promising technique for this purpose. Recent studies~\cite{zhu2023adfl,zhang2024badcleaner} have used model distillation to create robust student models that inherit the defense capabilities of the corresponding teacher model against backdoor attacks. We plan to look into this direction.


==> backup-tex/3-method-backup.tex <==
\section{GeminiGuard: DEFENDING AGAINST MPAS}
\label{sec:method-backup}
% In what follows, we first introduce the underlying intuitions and an overview of the FLBuff framework, followed by detailed descriptions of each component.
In this section, we first explain our idea of a comprehensive benchmarking framework in FL (Sect. \ref{subsec:design-niid-benchmark}), followed by key reasoning behind a unified approach towards tackling backdoor attacks amid \NIID data (Sect. \ref{subsec:design-uni-backdoor-niid}). We then introduce \FB as a concrete solution (Sect. \ref{subsec:design-fb}).

\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/small-buffer.pdf}
        \caption{With small buffer layer}
        \label{fig:small-buffer}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/large-buffer.pdf}
        \caption{With large buffer layer}
        \label{fig:large-buffer}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/feasibility-multi-attacks.pdf}
        \caption{Modelling different backdoors}
        \label{fig:multi-attack-feasibility}
    \end{subfigure}
    \vspace{-5pt}
    \caption{A unified view for modelling the impacts of backdoor attacks and Non-IIDs.}
    \label{fig:a-unified-view}
    \vspace{-5pt}
\end{figure*}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/small-vs-large-buffer.pdf}
%     \vspace{-2pt}
%     \caption{With and without sufficient buffer layer.}
%     \label{fig:flbuff-vs-others}
% \end{figure}



\subsection{A Comprehensive Benchmark for \NIID}
\label{subsec:design-niid-benchmark}

Here, we first work on benchmarking the performance of recent defenses against backdoor attacks under various \NIIDs in a systematic and comprehensive manner. Our goals are two-fold. First, we identify the lack of such a comprehensive evaluation benchmark for backdoor attacks (general MPAs as well) and defenses in FL, which is critical for future research in this field. Inspired by~\cite{li2022federated}, our aim is to provide a fair and easy-to-extend framework that researchers can conveniently evaluate and position their proposed MPAs including backdoors/MPA and/or novel defenses. Second, we want to better understand the current landscape of defenses against backdoor attacks on FL under comprehensive \NIIDs so as to figure out the key component for designing better defenses. 
%That is, we aim to identify the specific bottleneck resulting at the insufficiency of existing defenses. 
%is that the benchmark can shed light to inspirations for reliable defenses against MPAs under Non-iid. Meanwhile, we believe our effort here provides a good benchmark platform for evaluating both MPAs and defenses in a comprehensive and fair way.

To ensure that our benchmark is comprehensive, fair, and easy to use, we make sure that the solicited attacks, defenses, datasets, and ML tasks are diverse and representative so that the benchmark can be plugged-and-played for new attacks, defenses, datasets, and ML tasks. Table~\ref{tab:noniid_bechmark} shows the consolidated results of the baseline defenses used in this paper, where we make sure that the settings across different defenses are fair. While we defer the detailed settings to Section~\ref{eval:setup}, the overview is as follows. That is, the number of available clients is 100 while 10 out of them are to select in each training round. The number of backdoor attackers is 10, i.e., the backdoor ratio is 0.1. At each backdoor attacker, the data poisoning rate is 0.5.%, i.e., \ycnote{what does a poisoning rate of 0.5 mean?}.\nwnote{half of the training data are manipulated, half of the training data are benign}

We summarize two observations from Table~\ref{tab:noniid_bechmark} that lead us to deeper investigations of defenses under \NIIDs. More details can be found in Section~\ref{sec:evaluation:benchmark}:\\
\textbf{Observation 1.a:} The performance of most existing defenses under \NIIDs is much worse than that under IID. To some extent, these defenses are barely effective under \NIIDs. \\
\textbf{Observation 1.b:} At the very best, existing defenses may perform decently under one specific \NIID but none of them is close to working properly under two \NIIDs. Not to mention more complicated \NIIDs in practice. Given the necessity of practical and reliable defenses against backdoor attacks under various \NIIDs, it is by all means worthwhile to further the exploration of backdoor defenses that perform better from the perspectives of the above two observations.
%The results of MPAs and defenses under dir, qty, and prob on different datasets are shown in Table xxx. We summarize two findings from the results. On the one hand, the performance of a few defenses under Non-IID is not as what they're claimed to be. On the other hand, while some defenses are effective on dir (?), almost no existing defenses perform well under more than two Non-IID types. Given the necessity of reliable defenses against MPAs under Non-IID, it is by all means worthwhile to further the exploration of better MPA defenses.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/unified-view.pdf}
%     \vspace{-2pt}
%     \caption{A unified view for modelling the impact of backdoor attacks and Non-IIDs.}
%     \label{fig:unified-view}
% \end{figure}

\subsection{A Unified View for Backdoor Attacks and Non-IIDs} \label{sec:a-unified-view}%\xlnote{need to simplify this section}
\label{subsec:design-uni-backdoor-niid}
% Our ultimate goal is to find a single defense that works across backdoor attacks and \NIIDs, or even unknown attacks and unknown Non-IIDs. To start with, we conjecture the main reasons that lead to the above two observations from Table~\ref{tab:noniid_bechmark}. 

% Firstly, the main reason leading to degraded defense performance under one \NIID compared to IID is that (arbitrary) \NIID reduces the distinguishability between benign and malicious model updates. That is, benign model updates under IID \textit{can be} easily separated from malicious ones but benign model updates under even one \NIID \textit{cannot be} easily separated from malicious ones. This thus leads us to that \textit{if we can model the impact of (one or more) \NIIDs on the computed model update and that of backdoor under the same scope}, we may then be able to avoid or reduce the degradation of our defense from IID to \NIIDs. 

% Secondly, the main reason that very few existing defenses work for more than one \NIID is the general overlook of comprehensive \NIID settings. More importantly, existing defenses rarely took the fundamental impact of \NIIDs into their design process. Hence they may happen to work for one \NIID but seldom more of them. This thus leads us to a similar conclusion that \textit{if we can model the common impact of different \NIIDs on the computed model update}, we may then be able to design a single defense for different \NIIDs.
Our ultimate goal is to find a single defense that works across backdoor attacks and \NIIDs, or even unknown attacks and unknown Non-IIDs. To start with, we conjecture that the main reason leading to degraded defense performance under one \NIID compared to IID is that (arbitrary) \NIID reduces the distinguishability between benign and malicious model updates. That is, benign model updates under IID \textit{can be} easily separated from malicious ones but benign model updates under even one \NIID \textit{cannot be} easily separated from malicious ones. This thus leads us to that \textit{if we can model the impact of (one or more) \NIIDs on the computed model update and that of backdoor under the same scope}, we may then be able to avoid or reduce the degradation of our defense from IID to \NIIDs. we summarize the above observation into the following proposition:

%In addition, we conjecture that very few existing defenses work for more than one \NIID as few defenses explored the fundamental impact of \NIIDs and incorporated it into their design process. This thus leads us to that \textit{if we can model the common impact of different \NIIDs on the computed model update}, we may then be able to design a single defense for different \NIIDs.

%In this section, we aim to develop solid intuitions for our defense so that we can expect it to work under Non-IIDs. The ultimate goal is that we can find a single method/model that works across different MPAs and different Non-IIDs, or even unknown MPAs and unknown Non-IIDs. To that end, we anticipate the key questions to answer are ``Exactly what is the impact of Non-IID data distributions of a subset of benign clients on designing effective MPA defenses?'' and ``How about the impact of different MPAs on designing defenses effective on most/all of them?'' This leads us to Figure xxx and the following propositions.
% we summarize the above observation into the following proposition:
\begin{prop}
\label{prop:prior-defenses}
    Prior defenses against backdoor attacks in FL easily fail under \NIIDs because \NIIDs reduce the distinguishability between benign and malicious model updates.
\end{prop}

Next, we provide incremental reasoning toward the existence of a general approach to backdoor defense amid \NIID data.

% \begin{figure}[thb]
%     \centering
%     % Figure 1
%     \begin{subfigure}[b]{0.3\linewidth}
%         \includegraphics[width=\linewidth]{figures/noniid-degree/noniid_degree_ALIE.pdf}
%     \end{subfigure}
%     \hfill % This command inserts a space that adjusts between the side-by-side subfigures
%     % Figure 2
%     \begin{subfigure}[b]{0.3\linewidth}
%         \includegraphics[width=\linewidth]{figures/noniid-degree/noniid_degree_ALIE.pdf}
%     \end{subfigure}
%     \hfill
%     % Figure 3
%     \begin{subfigure}[b]{0.3\linewidth}
%         \includegraphics[width=\linewidth]{figures/noniid-degree/noniid_degree_ALIE.pdf}
%         % \caption{CIFAR-10}
%     \end{subfigure}
%     \caption{Inter-distance between PLRs in the 2-D space of the CIFAR10 dataset(class 0).}
%     \label{fig:cl_fl}
%     \vspace{-10pt}
% \end{figure}



\subsubsection{\NIID and Backdoor Attacks in Representation Space}
Figure~\ref{fig:small-buffer} illustrates a general situation where we map benign model updates under IID setting and malicious model updates (can be an arbitrary backdoor attack) into a representation space. Note that a node in such a space corresponds to a model update (either benign or malicious). The larger circle in green corresponds to the cluster of benign model updates from IID setting while the smaller circle in red corresponds to the cluster of malicious model updates from a certain backdoor attack. Provided the above setup, our first \textit{proposition for generic backdoor attacks} is that:
\begin{prop}
\label{prop:backdoor-1}
    For an arbitrary backdoor attack, its corresponding malicious model updates are obtained by moving nodes (see Figure~\ref{fig:small-buffer}) from the cluster of benign model updates under IID to as close as possible to optimal nodes determined by the goal (i.e., the optimization formulation) of the specific backdoor attack.
\end{prop}
In other words, the red circle (i.e., one backdoor attack) in Figure~\ref{fig:small-buffer} can be viewed as departing from the green circle (i.e., benign model updates under IID) \textit{along a defined optimal direction.} What's more, different backdoor attacks can be viewed as different red circles resulting from moving \textit{along different defined optimal directions,} which is our second corollary for backdoor attacks. 

\begin{corollary}
\label{cor:backdoor-2}
    Different backdoor attacks can be viewed as the results of moving nodes (see Figure~\ref{fig:multi-attack-feasibility}) from the same cluster of benign model updates under IID along different optimal directions, determined by each attack uniquely.
\end{corollary}

So far, we have modeled the behavior of backdoor attacks from the perspective of representation space. Surprisingly, we figure out that we can model the behavior of \NIIDs from the same perspective and the behaviors of backdoor attacks and \NIIDs are fundamentally different thus distinguishable. We first present our \textit{proposition for an arbitrary \NIID:}
\begin{prop}
\label{cor:niid-1}
    For an arbitrary \NIID, its corresponding benign model updates are simply expansion from the cluster of benign model updates under IID (see Figure~\ref{fig:small-buffer}). The angles and displacements are solely determined by the specific \NIID, hence resulting at different shapes for the cluster of benign model updates under different \NIIDs.
\end{prop}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.15\textwidth}
        \includegraphics[width=\textwidth]{figures/non-iid-a.pdf}
        \caption{\NIID, a}
        \label{fig:noniid-a}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
        \includegraphics[width=\textwidth]{figures/non-iid-b.pdf}
        \caption{\NIID, b}
        \label{fig:noniid-b}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
        \includegraphics[width=\textwidth]{figures/non-iid-c.pdf}
        \caption{\NIID, c}
        \label{fig:noniid-c}
    \end{subfigure}
    \vspace{-5pt}
    \caption{Examples of different \NIIDs in representation space.}
    \label{fig:noniids}
    \vspace{-5pt}
\end{figure}

Following that, our second corollary for \NIIDs is that: 
\begin{corollary}
\label{cor:niid-2}
    The cluster of benign model updates under different \NIIDs are simply different expansions from the cluster of benign model updates under IID (see three examples of \NIIDs in Figure~\ref{fig:noniids}) under different sets of angles and displacements, uniquely determined by each individual \NIID.
\end{corollary}

\subsubsection{\NIID v.s. Backdoor Attacks}
% Based on the above corollaries, we can better address \NIID challenges when designing defenses against backdoor attacks in FL. For instance, as can be seen in Figure~\ref{fig:small-buffer}, the reason that prior defenses failed under \NIID is that the expansion from \NIID leads to overlap between the cluster of benign model updates under \NIID and the cluster of malicious model update, hence degraded defense performance. More importantly, we come to our proposition featuring the difference between \NIID and backdoor attacks:
Based on the above corollaries, we can better address \NIID challenges when designing defenses against backdoor attacks in FL. For instance, as shown in Figure~\ref{fig:small-buffer}, prior defenses failed under \NIID simply because that the expansion from \NIID leads to overlap between the cluster of benign model updates under \NIID and the cluster of malicious model update. More importantly, we come to our proposition featuring the difference between \NIIDs and backdoor attacks:
\begin{prop}
\label{cor:niid-vs-backdoor}
    The impacts of \NIIDs and backdoor attacks are \textit{fundamentally} different: although they start from the same place (see Figure~\ref{fig:noniids}), \NIIDs are to expand in almost all directions while backdoor attacks are to depart in a single direction per attack.
\end{prop}
% Therefore, we conclude that \textit{theoretically there exist defense solutions against backdoor attacks that are not expected to be compromised by \NIIDs.} In practice, we believe that these solutions are likely simple because that expansion due to \NIIDs tends to result at \textit{smaller displacements with so many directions to expand}. On the contrary, the displacement from an arbitrary backdoor attack \textit{tends to be large} because that it has only one direction, i.e., the optimal direction, and the attack cluster needs to be sufficiently different from the benign cluster under IID in order to be malicious. As a result, we develop our first intuition for designing defenses that are effective under \NIIDs.
Given such a key difference, we conclude that \textit{theoretically there exist defense solutions against backdoor attacks that are not compromised by \NIIDs.} This is particularly true as in practice expansion due to \NIIDs tends to result at \textit{smaller displacements with so many directions to expand}. On the contrary, the displacement from an arbitrary backdoor attack \textit{tends to be large} because that it has only one direction, i.e., the optimal direction, and the attack cluster needs to be sufficiently different from the benign one \textit{in order to be malicious}. As a result, we develop our main intuition for designing defenses that are effective under \NIIDs.

\begin{figure}[t]
    \centering
    % Figure 1
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/plr-comparison/plr_iid.pdf}
    \end{subfigure}
    \hfill % This command inserts a space that adjusts between the side-by-side subfigures
    % % Figure 2
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/plr-comparison/plr_prob.pdf}
    \end{subfigure}
    \hfill
    % Figure 3
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\linewidth]{figures/plr-comparison/plr_flbuff.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=0.8\linewidth]{figures/plr-comparison/plr_legend.pdf} % Reduce the width if the legend is too large
    \end{subfigure}
    % \vspace{-5pt}
    \caption{Model updates for CIFAR-10 in PLR space under different scenarios: IID, \NIID (prob), and with \FB.}
    \label{fig:cl_fl}
    \vspace{-5pt}
\end{figure}

\textbf{Core Intuition:} The buffer layer between the cluster of benign model updates under IID and that of malicious model updates is the key component to decide how well the corresponding defense works under different \NIIDs. The larger buffer layer, the better defense even under different \NIIDs.

Figure~\ref{fig:small-buffer} and Figure~\ref{fig:large-buffer} together illustrate why the above intuition would hold. If a buffer layer is sufficiently large to cover even the expansion from one or more \NIIDs, the corresponding defense can perform well under \NIIDs. Figure~\ref{fig:cl_fl} illustrates how \FB can still work under \NIIDs. Particularly, we can see that on CIFAR-10, benign and malicious model updates under \NIID become less distinguishable when compared to those under IID while under \FB, they remain to be distinguishable. Besides, we have the following proposition regarding the possibility of using one defense against different backdoor attacks under different \NIIDs.

\begin{prop}
\label{cor:one-defense-for-all}
    The possibility that a single defense with a well-design buffer layer can be effective for more than one backdoor attack and more than one \NIID roots in that in representation space, different \NIIDs tend to be `similar' while different backdoor attacks tend to be quite `different' (see Figure~\ref{fig:multi-attack-feasibility}).
\end{prop}
We further elaborate on the above corollary here. In representation space, we term different \NIIDs to be `similar' by that the resulting clusters are expected to \textit{share the same centroid and overlap a lot}. This is because that while different \NIIDs differ in the expansion angles and displacements, they originate from the same cluster, i.e., the one of benign model updates under IID, and expansion displacements are small due to too many expansion angles. On the contrary, different backdoor attacks tend to be quite `different' simply because of their optimization formulations. Therefore, the resulting optimal directions would be quite different, plus they require larger displacements in order to be malicious. Combining the above two, hence a buffer layer that covers the expansion of one \NIID and separates one backdoor attack from the benign cluster is likely to cover the expansion of another \NIID and still separate another attack. As illustrated in Figure~\ref{fig:multi-attack-feasibility}, the buffer layer is expected to tackle not just attack $\mathcal{A}_1$ but $\mathcal{A}_2, \mathcal{A}_3,$ and $\mathcal{A}_4$ as well.

% \textbf{Proposition 1:} Why do prior defenses easily fail under Non-IIDs?

% \textbf{Proposition 2.1:} Non-IID is to expand benign representation in almost arbitrary direction.

% \textbf{Proposition 2.2:} Different Non-IIDs is to expand benign representation in almost arbitrary direction with different magnitude.

% \textbf{Proposition 3.1:} MPAs are to deviate from benign representation to the optimal malicious representation in almost a fixed direction.

% \textbf{Proposition 3.2:} Different MPAs are to deviate from benign representation to different optimal malicious representations in their unique (yet fixed) direction. See Figure xxx.

% \textbf{Intuition 1:} While prior defenses fail to work well under Non-IIDs, the impact of Non-IIDs and that of MPAs are still fundamentally different, hence granting opportunities for potential defenses that distinguish Non-IID benign and malicious well.

% Particularly, Non-IID expansion tends to be with smaller magnitude because of many directions to expand. The expansion or deviation magnitude of MPAs is doomed to be larger because they only have one direction, i.e., the optimal one, and MPAs need to be different from IID benign so as to be malicious.

% \textbf{Intuition 2:} Buffer is all you need.

% \textbf{Emphasize that such a unified view provides the foundation for better future defenses.}

\subsection{GeminiGuard: Buffer is All You Need}
\label{subsec:design-fb}
% Based on the above intuition, the core design of \FB is to create a sufficiently large buffer layer in the representation space between the cluster of benign updates under IID and that of malicious updates. Such a design has the potential to work across different backdoor attacks and different \NIIDs. Meanwhile, we believe that the above unified view of backdoor attacks and \NIIDs can serve to provide the foundation for better future defenses. 

% To that end, we decide to design \FB as an aggregation-based defense which uses penultimate layer representations (PLRs) to denote model updates from remote clients (as in FLARE~\cite{wang2022flare}) and a supervised contrastive learning model to further train better representations from labelled PLRs. Particularly, the learned representations are expected to further maximize the distance between benign and malicious PLRs while minimizing the distances among benign PLRs and among malicious PLRs. 
Based on the above intuition, the core design of xxxx is to create a sufficiently large buffer layer in the representation space between the cluster of benign updates under IID and that of malicious updates. To that end, we design xxxx as an aggregation-based defense which uses penultimate layer representations (PLRs) to denote model updates from remote clients and a supervised contrastive learning model to further train better representations from labelled PLRs. Particularly, the learned representations are expected to further maximize the distance between benign and malicious PLRs while minimizing the distances among benign PLRs and among malicious PLRs, hence effectively enlarging the buffer layer. 


\textbf{Step 1:} As in typical FL process, a client $u_i$ needs to send her model update after local training to PS. Specifically, $u_i$ first receives global model $\Theta$ from PS and uses it to initialize her local model $\mathbf{\theta}_i$. $u_i$ then trains $\mathbf{\theta}_i$ using her local data and uploads model update $\delta_i$ to PS.

\textbf{Step 2:} \FB is txo compute the corresponding PLR sequence for each received model update. Following {CrowdGuard}~\cite{CrowdGuard}, we assume that PS has a small set of auxiliary IID data (denoted by $D_A$) for assisting \FB against backdoor attacks. Given $\delta_i$, {\FB first aggregates the current $\Theta$ and $\delta_i$ together and obtains $\Theta_i$.} The corresponding PLR sequence of $\delta_i$ can be readily obtained by feeding $D_A$ to $\Theta_i$ and then extracting the per-sample representations at penultimate layer, i.e., the second last layer, and concatenating them one by one. For instance, assuming that the mapping function of $\Theta_i$ is $g_{\Theta_i}:x\in \mathcal{R}^{l \times w \times h} \rightarrow r \in \mathcal{R}^{p}$ where $l, w$, and $h$ denote the width, height, and channels of an image input, respectively, and $p$ the size of PLR. Assume that $D_A$ has $m$ data records, the PLR sequence of $\delta_i$ is thus $\text{PSeq}_i =: \{g_{\Theta_i}(x_1),\ldots,g_{\Theta_i}(x_m)\}$.

\textbf{Step 3:}

==> backup-tex/4-evaluation-backup.tex <==
\section{Performance Evaluation}
\label{sec:evaluation-backup}
% In this section, we evaluate FLBuff from the following aspects.
In this section, we focus on evaluating the performance of FLBuff under five Non-IIDs. We also conduct an ablation study to demonstrate FLBuff's applicability across different backdoor attacks and different \NIIDs. Subsequently, we investigate the impact of various parameters on FLBuff. Finally, we evaluate FLBuff against comprehensive adaptive attacks.

\subsection{Experimental Settings}
\label{eval:setup}

\subsubsection{Implementation} 
Our experiments were implemented in Python using PyTorch. The experiments were executed on a server with an Intel(R) Core(TM) i9-10900X CPU @ 3.70GHz, two NVIDIA RTX 3090 GPUs, and 181 GB main memory. Meanwhile, the source code for FLBuff including the benchmark for \NIIDs is available at \url{https://anonymous.4open.science/r/FLBuff-32B4/}. 

\subsubsection{Datasets} 
\label{non-iid-datasets}
We evaluated \FB on three image datasets and one text dataset. For image classification task, we use three popular benchmark datasets MNIST~\cite{deng2012mnist}, Fashion-MNIST(FMNIST)~\cite{xiao2017fashion}, and CIFAR10~\cite{cifar10}. Each of the three datasets contains samples from 10 classes and are frequently used for evaluations of backdoor attacks as well as defenses ~\cite{abadi2016deep,wang2022flare,zhangfldetecotr,CrowdGuard}. We use the IMDB dataset~\cite{imdb} for sentiment analysis task. It contains 50,000 movie reviews split equally between training and testing sets. 

We considered IID and five \NIIDs in this paper. For IID scenarios, we divide the data equally among clients. For non-IID scenarios, we consider five \NIID types with the following default parameters: \textbf{1)} prob-based with a non-IID degree of 0.3, \textbf{2)} dir-based with a non-IID degree of 0.3,  \textbf{3)} qty-based where each client only has two classes, \textbf{4)} noise-based feature distribution skew with $\sigma=0.5$, and \textbf{5)} quantity skew with $\beta=0.5$ for Dirichlet distribution.  Aside from the above, we also explore different \NIID degrees in ablation study to evaluate their impacts on the effectiveness of \FB at Sect.~\ref{noniid-degree-study} and Appendix~\ref{sec:appenddix-additional-results}.

%\ycnote{Aside the default settings, we also evaluate the impact of \NIID degree in prob-based and dir-based and the number of classes in qty-based.}\xlnote{In evaluating the impact of \NIID, we normalized and scaled the non-iid degree of these three \NIIDs to a range of 0.1 to 0.9, with higher values indicating more severe non-iid conditions.}

\begin{table}[!ht]
    
    \renewcommand{\arraystretch}{1.3}
    \centering
    \footnotesize
    % \small
    \caption{Datasets and models used in \FB.}
    \label{tab:pros_dataset}
    \begin{tabular}{p{1.6cm}|p{1.2cm}p{1.2cm}p{1cm}p{1.8cm}}
        \hline
        Dataset (\# of categories) & \# of training samples  & \# of testing samples & \# of input size & \# of Model architecture $\Theta$ \\ 
        \hline
        MNIST (10) & 60,000 & 10,000 & (28, 28, 1) & 3 Blocks + 6 Conv\\
        FMNIST (10) & 60,000 & 10,000 & (28, 28, 1) & 3 Blocks + 6 Conv\\
        CIFAR10 (10) & 50,000 & 10,000 & (32, 32, 3) & ResNet-50\\
        IMDB (2) & 40,000 & 10,000 & (100,) & LSTM\\
        \hline
    \end{tabular}
    \vspace{-10pt}
\end{table}

\subsubsection{FL Settings} 
%We run the training for 20 global rounds in each FL training. 
In each FL round, we select 10 clients out of a total of 100 clients to participate FL training. By default, the malicious client ratio is set to 0.1, and the data poisoning rate is 0.5. Eeach selected client trains its local model using a batch size of 64 for five local epochs before aggregating the updates. {The classification threshold is set to 0.5 for the Sup-CL model.} For MNIST and FMNIST datasets, we adopt cross-entropy as the loss function, stochastic gradient descent (SGD) optimizer with a learning rate of 0.001, and a momentum of 0.9 to train models. For CIFAR10 dataset, we use the same loss function, optimizer, and momentum decade but adopt a learning rate of 0.01 for SGD instead. Finally, for IMDB dataset, we adopt cross-entropy with logit as the loss function and Adam optimizer with a learning rate of 0.001.

\subsubsection{Models} We adopt a CNN model for MNIST and FMNIST datasets while ResNet-50 for CIFAR10. For IMDB dataset, we use an LSTM network to handle sequential text data. These models are shown in Table~\ref{tab:pros_dataset} while more details can be found in Appendix~\ref{sect:appendix-model}. 

\subsubsection{Metrics}
%\nwnote{detection accuracy and model accuracy are with the same notion.}
We use the following metrics to evaluate FLBuff:
\begin{itemize}
    %\item Detection accuracy $\texttt{Acc}$ which denotes the ratio of correctly predicted samples among the testing set regardless of benign or malicious. The higher $\texttt{Acc}$, the better performance.
    \item Attack success rate (\texttt{ASR}) which denotes the ratio of backdoor samples among the backdoor testing set that successfully receive targeted predictions from the victim FL model. The lower \texttt{ASR}, the better performance an arbitrary defense including \FB provides.
    \item Model accuracy (\texttt{Acc}) which denotes the testing accuracy of the targeted FL model (i.e., the victim model) during the testing phase. The higher \texttt{Acc}, the better model performance.
\end{itemize}

\subsubsection{Backdoor Attacks and Defense Baselines} 
\label{sec:attacks-and-defenses-used}

We evaluate \FB against four powerful and stealthy backdoor attacks: \textit{BadNet}~\cite{gu2017badnets}, \textit{DBA}~\cite{xie2019dba}, \textit{Scaling}~\cite{bagdasaryan2020backdoor}, and \textit{ALIE}~\cite{baruch2019little} and compare it to five SOTA defenses against backdoor attacks: \textit{FLTrust}~\cite{cao2021fltrust}, \textit{FLDetector}~\cite{zhangfldetecotr}, \textit{FLARE}~\cite{wang2022flare}, \textit{FLAME}~\cite{nguyen2022flame}, and \textit{FLIP}~\cite{zhang2023flipprovabledefenseframework}. Due to space limits, we retain the details of the above attacks and defenses in the Appendix~\ref{sec:appendix-attacks}.
% We use the following five SOTA defenses against backdoor attacks as the baselines for FLBuff.
% % \item \textbf{Krum and Multi-Krum}: these methods select updates closest to the majority to minimize the influence of malicious updates.
% \begin{itemize}
%     \item \textit{FLTrust}~\cite{cao2021fltrust} used a small trusted dataset to assign trust scores and normalize model updates from clients, hence reducing the impact of malicious updates.
%     \item \textit{FLDetector}~\cite{zhangfldetecotr} focused on detecting and removing malicious clients by checking the consistency of a client's model updates across multiple training rounds.
%     \item \textit{FLARE}~\cite{wang2022flare} proposed to compute trust scores for model updates using representations in order to distinguish between malicious and benign updates, hence providing robust aggregation under backdoor attacks.
%     \item \textit{FLAME}~\cite{nguyen2022flame} combined model update clustering, weight clipping, and noise injection together to eliminate the impact from backdoor attacks.
%     \item \textit{FLIP}~\cite{zhang2023flipprovabledefenseframework} proposed to better model robustness against backdoor attacks through reverse engineering the triggers from attacks.
% \end{itemize}
Note that we anticipate that \FB is highly likely to work under other backdoor attacks and model poisoning attacks as well. Our benchmark framework for \NIID evaluations can incorporate future defenses readily as well.

% \subsubsection{Default Parameters and Evaluation Goals}
% We highlight the default hyperparameters here for clarity purpose. The size of a query is $N_b=200$ while the total sequence length, i.e., the total query samples, is $l=2,000$. Our main evaluation goals from the below experiments are (1) FLBuff achieves a high accuracy confirming , (2) FLBuff achieves a high accuracy, and (3) FLBuff achieves a higher detection rate on both known and unknown MPAs. 
\subsection{Evaluation Goals}
%Our main evaluation goals from the below experiments are 
%(1) FLBuff achieves a high accuracy confirming , (2) FLBuff achieves a high accuracy, and (3) FLBuff achieves a higher detection rate on both known and unknown backdoor attacks. 
{
We introduce our evaluation goals here to make the following experimental results easier to follow:  
\textbf{Goal 1:} providing comprehensive attack and defense benchmarks under multiple \NIID settings, \textbf{Goal 2:} evaluating the effectiveness of FLBuff, \textbf{Goal 3:} exploring how the knowledge of partial malicious strategies can enhance defense performance, \textbf{Goal 4:} exploring how the knowledge of partial \NIIDs can enhance the defense performance, and finally \textbf{Goal 5:} evaluating defense effectiveness under various factors. }

Evaluation \textbf{Goal 2} and \textbf{Goal 5} are straightforward as shared with the literature. We elaborate on the reasons for designing the other three goals as follows. {\textbf{Goal 1} is critical as SOTA defenses do not consider \NIID data or only one \NIID setting. We aim to evaluate if the defenses proposed for IID data are effective under \NIID scenarios and if the defenses proposed for one \NIID data are effective under other \NIID settings. It would be great if we could design a defense that works well for multiple attacks while assuming no knowledge of the attack and no knowledge of \NIID data. Based on our evaluations below, no such defense has been provided yet. Given that recent literature has provided a tremendous amount of intelligence in attack domains, thus it is natural to consider how known attacks could help design a more effective defense against novel attacks. For this purpose, we designed \textbf{Goal 3}, where one or more attacks are provided in the defense designing phase, and unseen attacks are evaluated in the defense testing phase. Similarly, in \textbf{Goal 4}, one or more \NIID types are provided in the defense designing phase, and unseen \NIIDs are tested in the defense evaluation phase to investigate how much performance gain these known \NIIDs can introduce. }

%The results reveal that the SOTA defenses perform poorly on some \NIID partitions and exhibit significant variation across different \NIID partitions. For instance, the FLTrust defense exhibits \texttt{ASR} ranging from 0.46\% to 79.07\% across different datasets and \NIIDs, indicating inconsistency in performance against backdoor attack.

\begin{table*}[ht]
\centering
% \scriptsize
\renewcommand{\arraystretch}{1.2} 
\caption{\texttt{ASR} (\%) of backdoor attacks with SOTA defenses under various Non-IID settings.}
\label{tab:noniid_bechmark}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|cccccc|cccccc|cccccc|cccccc}
\hline
\multirow{2}{*}{\textbf{Defense}} & \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{6}{c|}{\textbf{BadNet}} & \multicolumn{6}{c|}{\textbf{DBA }} & \multicolumn{6}{c}{\textbf{Scaling }} & \multicolumn{6}{c}{\textbf{ALIE }} \\
\cline{3-26}
 &  & \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty} & \textbf{noise} & \textbf{qs}  & \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty} & \textbf{noise} & \textbf{qs} & \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty} & \textbf{noise} & \textbf{qs} & \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty} & \textbf{noise} & \textbf{qs}  \\
\hline
% \multirow{3}{*}{Krum} & MNIST & 99.8 & 100.0 & 99.0 & 98.9 & 97.8 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 99.9 & 97.6 &  100.0 &  100.0 \\
%  & FMNIST & xx & xx & xx & xx & xx & xx & xx & xx & xx & \textcolor{red}{xx} & xx & xx & & & &  \\
%  & CIFAR10 & xx & \textcolor{red}{xx} & \textcolor{red}{xx} & xx & xx & xx & \textcolor{red}{xx} & xx & xx & xx & \textcolor{red}{xx} & \textcolor{red}{xx} & & & &  \\
%   & IMDB & xx & \textcolor{red}{xx} & \textcolor{red}{xx} & xx & xx & xx & \textcolor{red}{xx} & xx & xx & xx & \textcolor{red}{xx} & \textcolor{red}{xx} & & & &  \\
% \midrule
% \multirow{3}{*}{Multi-Krum} & MNIST & xx & xx & xx & xx & xx & xx & xx & xx & xx & xx & xx & xx & & & &  \\
%  & FMNIST & xx & \textcolor{red}{xx} & xx & xx & xx & xx & xx & \textcolor{red}{xx} & xx & \textcolor{red}{xx} & \textcolor{red}{xx} & \textcolor{red}{xx}& & & &   \\
%  & CIFAR10 & xx & \textcolor{red}{xx} & \textcolor{red}{xx} & xx & xx & \textcolor{red}{xx} & xx & xx & xx & \textcolor{red}{xx} & xx & \textcolor{red}{xx} & & & &  \\
%   & IMDB & xx & \textcolor{red}{xx} & \textcolor{red}{xx} & xx & xx & xx & \textcolor{red}{xx} & xx & xx & xx & \textcolor{red}{xx} & \textcolor{red}{xx} & & & &  \\
%  \midrule
\multirow{3}{*}{\textbf{FLTrust}}
    & MNIST & 0.90 & 2.01 & 2.70 & 4.99 & 1.70 & 8.16 & 0.78 & 2.25 & 3.29 & 6.12  & 3.12 & 10.75 & 0.46 & 4.17 & 3.20 & 10.96  & 2.40 & 9.71 & 0.84 & 4.51 & 5.02 & 6.61 & 2.42 & 10.85\\
    & FMNIST & 0.63 & 4.07 & 3.03 & 7.36  & 2.90 & 10.24 & 1.46 & 4.59 & 6.20 &  8.50 & 3.20 & 9.57 & 2.80 & 3.87 & 5.38 & 11.88  & 5.00 & 8.40 & 0.78 & 3.42 & 2.01 & 8.55 & 4.84 & 7.26 \\
    & CIFAR10 & 2.51 & 10.09 & 7.12 & 10.80  & 5.72 & 13.44 & 1.25 & 8.71 & 7.73 & 13.39 & 8.33 & 10.62 & 0.89 & 13.21 & 7.70 & 15.31  & 4.32 & 48.01 & 0.94 & 11.29 & 8.79 & 17.54 & 6.18 & 12.35 \\
    & IMDB & 3.09 & 10.22 & 13.17 & 10.75  & 5.40 & 11.60 & 4.03 & 7.35 & 8.04 & 11.01  & 4.50 & 12.57 & 3.27 & 7.09 & 10.55 & 9.15  & 3.90 & 11.27 & 4.23 & 9.47 & 7.41 & 10.31 & 5.91 & 13.88 \\
    \hline
\multirow{3}{*}{\textbf{FLARE}} 
    & MNIST & 0.48 & 3.10 & 2.77 & 2.40  & 2.08 & 12.42 & 0.42 & 2.27 & 2.52 & 0.94  & 3.44 & 8.14 & 0.52 & 1.25 & 2.92 & 5.56  & 3.79 & 10.12 & 0.32 & 6.57 & 5.01 & 7.91 & 3.34 & 8.66 \\
    & FMNIST & 1.00 & 7.10 & 5.80 & 7.31  & 5.97 & 14.43 & 4.40 & 5.90 & 6.92 & 4.25  & 5.17 & 10.03 & 4.72 & 15.80 & 2.90 & 6.98  &  5.43 & 15.45 & 0.10 & 7.31 & 8.19 & 10.05 & 3.30 & 12.91 \\
    & CIFAR10 & 1.80 & 10.81 & 6.90 & 9.77  & 10.10 & 20.01 & 1.50 & 10.40 & 13.10 & 3.72  &  10.80 & 17.90 & 2.10 & 11.60 & 12.60 & 8.89  & 10.97  & 13.50 & 1.14 & 12.06 & 13.56 & 8.45 & 9.45 & 18.61 \\
    & IMDB & 2.47 & 10.06 & 6.17 & 11.57  & 9.30 & 11.20 & 2.92 & 8.89 & 10.22 & 6.98  & 12.30 & 14.40 & 1.91 & 7.54 & 8.18 & 8.95  & 8.56 &  12.30 & 2.81 & 5.52 & 10.20 & 11.13 & 9.90 & 12.10 \\
    \hline
\multirow{3}{*}{\textbf{FLDetector}} 
    & MNIST & 0.26 & 8.80 & 5.96 & 10.54  & 1.10 & 10.22 & 1.53 & 3.41 & 8.96 & 12.51  & 1.57 & 6.39 & 2.01 & 4.60 & 4.19 & 16.52  & 2.79 & 10.58 & 0.95 & 5.17 & 5.30 & 8.90 & 3.78 &  10.92 \\
    & FMNIST & 0.29 & 9.14 & 4.28 & 12.05  & 2.70 & 15.25 & 3.89 & 4.13 & 6.51 & 15.43  &  5.00 & 11.10 & 2.89 & 7.00  & 5.90 & 18.74  & 3.60 & 15.34 & 1.87 & 5.52 & 4.13 & 12.78  & 4.93 & 14.10 \\
    & CIFAR10 & 3.26 & 8.42 & 8.31 & 16.50  & 10.10 & 14.90 & 3.43 & 10.57 & 8.24 & 15.50  & 8.70 & 22.60 & 6.60 & 7.08 & 5.10 & 16.95  & 10.02  & 27.88 & 1.93 & 9.29 & 5.41 & 10.93 & 8.50 & 35.80\\
    & IMDB & 3.15 & 6.10 & 5.30 & 19.25  & 9.68 & 16.54 & 2.82 & 7.52 & 5.46 & 18.83  &  5.72 & 25.52 & 3.02 & 5.46 & 5.02 & 7.51  & 8.10 & 10.90 & 4.70 & 7.35 & 6.23 & 8.50 & 5.40 & 10.90\\
   \hline
\multirow{3}{*}{\textbf{FLAME}} 
    & MNIST & 0.21 & 1.35 & 3.37 & 3.32  & 0.63 & 2.29 & 0.30 & 1.46 & 1.88 & 1.48  & 0.31 & 3.96 & 0.44 & 1.71 & 5.18 & 1.64  & 1.88 & 5.11 & 0.28 & 1.52 & 2.82 & 3.85 & 0.94 & 5.66 \\
    & FMNIST & 0.75 & 2.10 & 6.58 & 7.86  & 1.52 & 8.10 & 0.43 & 3.30 & 3.55 & 4.53  & 3.64 & 7.24 & 0.91 & 5.51 & 8.23 & 6.15  & 4.37 & 6.10 & 1.74 & 5.70 & 6.72 & 5.60 & 2.10 & 8.00 \\
    & CIFAR10 & 3.20 & 5.10 & 6.50 & 11.10  & 7.80 & 18.60 & 3.30 & 10.60 & 7.70 & 14.51  &  6.50 & 11.80 & 1.80 & 10.60 & 6.80 & 10.72  & 4.10 &  11.00 & 1.15 & 7.80 & 10.70 & 11.25 & 2.73 &  14.50 \\
    & IMDB & 1.02 & 3.35 & 7.15 & 9.90  & 5.80 & 10.00 & 1.63 & 6.45 & 10.68 & 9.95  & 4.83 & 9.64 & 2.07 & 8.55 & 6.73 & 10.16  & 6.10 & 10.10 & 2.12 & 8.75 & 6.85 & 10.30 & 3.00 & 10.60 \\
    \hline
\multirow{3}{*}{\textbf{FLIP}} 
    & MNIST & 1.13 & 5.11 & 7.27 & 8.32  & 1.42 & 4.87 & 2.10 & 10.82 & 11.4 & 12.38  & 5.35 & 2.44 & 1.22 & 5.53 & 8.98 & 9.54  & 2.10 &  4.68 & 3.21 & 8.65 & 12.52 & 8.75 & 3.85 & 7.51 \\
    & FMNIST & 0.30 & 4.98 & 4.58 & 10.76  & 2.71 & 5.38 & 4.14 & 10.41 & 8.85 & 12.63  & 1.24 & 6.90 & 1.11 & 12.36 & 9.13 & 9.05  & 0.73  &  5.97 & 2.14 & 7.36 & 8.82 & 8.70 & 4.90 & 4.83 \\
    & CIFAR10 & 3.20 & 8.78 & 9.90 & 14.30  & 6.88 & 24.20 & 6.60 & 7.44 & 8.80 & 10.61  & 12.70 & 27.90 & 5.60 & 8.69 & 7.90 & 10.81  & 7.20 & 15.40 & 1.45 & 10.91 & 11.10 & 14.35 & 9.00 & 21.80\\
    & IMDB & 3.12 & 9.45 & 10.25 & 12.00  & 4.50 & 10.20 & 5.73 & 13.55 & 7.78 & 12.05  & 5.45 & 11.70 & 2.17 & 21.65 & 22.83 & 13.26  & 3.70 & 8.40 & 3.22 & 11.85 & 9.95 & 13.40 & 6.20 & 15.30 \\ 
    \hline
\multirow{3}{*}{\textbf{FLBuff}} & MNIST & 0.30 & 1.00 & 0.70 & 0.52  & 0.98 & 0.65 & 0.56 & 1.27 & 0.90 & 1.40  & 0.70 & 0.85  & 0.15 & 0.12 & 0.43 & 0.28  & 0.71 & 0.60 & 0.93 & 1.07 & 1.25 & 0.42 & 1.14 & 0.53 \\
     & FMNIST & 0.85 & 0.53 & 0.87 & 1.23  & 0.53 & 0.51 & 0.15 & 0.25 & 0.47 & 0.22  & 1.12 & 0.49 & 0.62 & 0.31 & 0.92 & 0.76  & 0.65 & 0.81 & 0.76 & 0.74 & 0.38 & 1.07 & 0.95 & 0.85  \\
     & CIFAR10 & 1.30 & 1.28 & 0.94 & 0.77  & 1.40 & 1.22  & 0.51 & 0.93 & 0.55 & 1.42  & 1.19  & 0.65 & 0.35 & 1.13 & 0.77 & 0.81  & 0.54 & 1.20 & 0.04 & 0.19 & 1.26 & 1.01 & 0.68 & 1.09 \\
     & IMDB & 0.62 & 0.33 & 0.89 & 1.10  & 1.18 & 0.94 & 0.35 & 1.18 & 0.50 & 0.60  & 0.74 & 0.70 & 0.85 & 1.26 & 0.93 & 1.05 & 0.72 & 1.05 & 0.97 & 0.22 & 0.29 & 0.86 & 0.84 & 0.91 \\
\hline
\end{tabular}
}
\end{table*}
% \multirow{3}{*}{\textbf{FLTrust}} 
%     & MNIST & 0.90 & \underline{\textbf{39.01}} & 24.70 & 51.99 & 0.78 & 30.25 & 10.29 & 27.12 & \underline{\textbf{0.46}} & 10.17 & 9.20 & 15.96 & 0.84 & 7.51 & 25.02 & 20.61 \\
%     & FMNIST & 0.63 & \underline{\textbf{79.07}} & 19.03 & 49.36 & 6.46 & 9.59 & 10.20 & 29.39 & 2.80 & 11.87 & 13.38 & 45.88 & 0.78 & 10.42 & 30.01 & 22.55 \\
%     & CIFAR10 & 2.51 & \underline{\textbf{26.09}} & 65.12 & 33.80 & 1.25 & 18.71 & 7.73 & 29.52 & 0.89 & 33.21 & 47.70 & 25.31 & 0.94 & 21.29 & 28.79 & 17.54 \\
%     & IMDB & 11.09 & \underline{\textbf{24.22}} & 23.17 & \underline{\textbf{37.75}} & 9.03 & 27.35 & 43.04 & 36.01 & 6.27 & 47.09 & 50.55 & 33.15 & 10.23 & 26.47 & 17.41 & 28.31 \\
%     \hline
% \multirow{3}{*}{\textbf{FLARE}} 
%     & MNIST & 0.48 & \underline{\textbf{0.10}} & 2.77 & 2.40 & 0.42 & 0.27 & 2.52 & 0.94 & 0.52 & 1.25 & 2.92 & 20.56 & 0.32 & 6.57 & 15.01 & 9.91 \\
%     & FMNIST & 1.00 & \underline{\textbf{15.10}} & 24.80 & 74.31 & 4.40 & 3.90 & 6.92 & 12.25 & 4.72 & 15.80 & 2.90 & 2.98 & 0.10 & 17.31 & 28.19 & 13.05 \\
%     & CIFAR10 & 8.80 & \underline{\textbf{18.81}} & 6.90 & 24.77 & 9.50 & 20.40 & 13.10 & 3.72 & 6.10 & 91.60 & 42.60 & 12.89 & 1.14 & 12.06 & 13.56 & 18.45 \\
%     & IMDB & 6.47 & \underline{\textbf{11.06}} & 16.17 & \underline{\textbf{31.57}} & 2.92 & 18.89 & 17.22 & 13.98 & 4.91 & 17.54 & 28.18 & 15.95 & 2.81 & 20.52 & 28.18 & 41.13 \\
%     \hline
% \multirow{3}{*}{\textbf{FLDetector}} 
%     & MNIST & 0.26 & \underline{\textbf{28.80}} & 13.96 & 66.54 & 3.53 & 33.41 & 8.96 & 62.51 & 3.53 & 64.60 & 11.19 & 66.52 & 0.95 & 19.17 & 25.30 & 18.90 \\
%     & FMNIST & 0.29 & \underline{\textbf{39.14}} & 13.28 & 68.05 & 3.89 & 64.13 & 6.51 & 65.43 & 2.89 & 38.90 & 25.00 & 18.74 & 1.87 & 18.52 & 25.13 & 12.78 \\
%     & CIFAR10 & 8.26 & \underline{\textbf{18.42}} & 38.31 & 16.50 & 8.43 & 10.57 & 8.24 & 31.50 & 6.60 & 27.08 & 31.10 & 26.95 & 1.93 & 9.29 & 15.41 & 10.93 \\
%     & IMDB & 8.15 & \underline{\textbf{28.10}} & 32.20 & \underline{\textbf{19.25}} & 7.82 & 27.52 & 32.46 & 18.83 & 10.02 & 31.46 & 23.02 & 37.51 & 7.70 & 27.35 & 31.23 & 18.50 \\
%    \hline
% \multirow{3}{*}{\textbf{FLAME}} 
%     & MNIST & 2.53 & \underline{\textbf{17.11}} & 6.37 & 25.32 & 6.60 & 16.92 & 19.88 & 70.48 & 5.30 & 12.73 & 6.18 & 71.64 & 2.81 & 10.55 & 10.82 & 15.85 \\
%     & FMNIST & 0.10 & \underline{\textbf{12.88}} & 10.58 & 37.86 & 3.04 & 20.31 & 13.55 & 49.53 & 0.91 & 10.26 & 8.23 & 56.15 & 1.74 & 15.25 & 16.72 & 15.60 \\
%     & CIFAR10 & 8.10 & \underline{\textbf{28.68}} & 8.90 & 11.20 & 10.01 & 22.34 & 7.70 & 34.51 & 7.80 & 55.59 & 6.80 & 75.72 & 10.15 & 28.82 & 19.00 & 11.25 \\
%     & IMDB & 3.02 & \underline{\textbf{20.35}} & 27.15 & \underline{\textbf{19.90}} & 1.63 & 17.45 & 17.68 & 19.95 & 5.07 & 18.55 & 21.73 & 30.16 & 2.12 & 28.75 & 16.85 & 30.30 \\
%     \hline
% \multirow{3}{*}{\textbf{FLIP}} 
%     & MNIST & 6.13 & \underline{\textbf{20.11}} & 17.27 & 28.32 & 5.10 & 10.82 & 41.4 & 32.38 & 1.22 & 15.53 & 25.98 & 29.54 & 3.21 & 28.65 & 22.52 & 18.75 \\
%     & FMNIST & 0.30 & \underline{\textbf{14.98}} & 11.58 & 40.76 & 4.14 & 23.41 & 15.85 & 12.63 & 1.11 & 12.36 & 9.13 & 29.05 & 2.14 & 17.36 & 18.82 & 18.70 \\
%     & CIFAR10 & 12.20 & \underline{\textbf{21.78}} & 29.90 & 14.30 & 12.21 & 25.44 & 28.80 & 17.61 & 8.90 & 28.69 & 47.90 & 38.81 & 1.45 & 30.91 & 21.10 & 14.35 \\
%     & IMDB & 8.12 & \underline{\textbf{23.45}} & 30.25 & \underline{\textbf{22.00}} & 9.73 & 23.55 & 20.78 & 22.05 & 9.17 & 21.65 & 22.83 & 13.26 & 3.22 & 31.85 & 19.95 & 23.40 \\ 
%     \hline
% \multirow{3}{*}{\textbf{FLBuff}} & MNIST & \underline{\textbf{0.30}} & \underline{\textbf{1.00}} & \underline{\textbf{0.70}} & \underline{\textbf{0.52}} & 0.56 & 1.27 & 0.90 & 1.40 & 0.15 & 0.12 & 0.43 & 0.28 & 0.93 & 1.07 & 1.25 & 0.42  \\
%      & FMNIST & 0.85 & \underline{\textbf{0.53}} & 0.87 & 1.23 & 1.12 & 0.25 & 0.47 & 0.22 & 0.62 & 0.31 & 0.92 & 0.76 & 0.96 & 0.74 & 0.38 & 1.07  \\
%      & CIFAR10 & 1.30 & \underline{\textbf{1.28}} & 0.94 & 0.77 & 1.19 & 0.93 & 0.55 & 1.42 & 0.35 & 1.13 & 0.77 & 0.81 & 0.04 & 0.19 & 1.26 & 1.01 \\
%      & IMDB & 0.62 & \underline{\textbf{0.33}} & 0.89 & \underline{\textbf{1.10}} & 0.35 & 1.18 & 0.50 & 0.73 & 0.85 & 1.26 & 0.93 & 1.05 & 0.97 & 0.22 & 0.29 & 0.86  \\
% \hline
% \end{tabular}
% \end{table*}

\subsection{Experimental Results}
\subsubsection{Non-IID Benchmark} \label{sec:evaluation:benchmark}
% We show \texttt{ASR} of the above SOTA defenses against the four backdoor attacks across multiple datasets and different Non-IID settings in Table~\ref{tab:noniid_bechmark}.

Table~\ref{tab:noniid_bechmark} shows the \texttt{ASR} of five SOTA defenses against four backdoor attacks under both IID and five \NIIDs. Our first finding is that existing defenses are not as robust as claimed when evaluated across different Non-IID scenarios. For most defenses, their performance drop significantly when the scenario goes from IID to an arbitrary \NIID type. For instance, \texttt{ASR} of FLTrust under \NIIDs changes vastly between 0.46\% to 48.01\%. This indicates that \NIID reduces the distinguishability of malicious updates from benign ones in the eyes of prior defenses. {Our second finding reveals that while certain defenses may remain effective under a specific \NIID type, it is rare for a defense to perform well across all \NIIDs evaluated}. One possible reason is the lack of built-in design for addressing \NIIDs in these defenses therefore it is difficult to tell their applicability. In comparison, \FB achieves the best performance among all.


\subsubsection{Performance of FLBuff}
\label{sec:evaluation:flbuff}

% Figure~\ref{fig:att} shows \texttt{ASR} of the above MSAs we obtained from different datasets, which is consistent to that in. The results indicate that these attacks are able to achieve, thus necessitating reliable defenses for. \xl{The attack success rate is based on a specific model,this part result is the same with Applicability to other MPAs under other Non-IIDs? .}
Here we first explore the setting that \FB is applied for defending against the same backdoor attack that it is trained for, i.e., we use the labelled samples from one backdoor attack to train a \FB model and then use the trained model for defending against the same attack. For instance, in Table~\ref{tab:apply_to_non_iid}, when \FB trained from labelled data under IID and BadNet attack on MNIST and then used for defending against BadNet, the obtained ASR when the testing scenario is IID, dir, prob, qty, noise, and qs is 1.82\%, 9.73\%, 10.04\%, 10.76\%, 1.90\%, and 6.55\%, respectively. Note that the results are obtained from a single \FB model. Essentially, this corresponds to the above \textbf{Goal 2}, in which we want to confirm whether a trained \FB model under IID can be effective under the five \NIIDs or not. If the answer is `yes', it indicates that at least a trained \FB model can defend against the same backdoor attack it trains from, particularly under various \NIIDs. This is important in practical as we, as the defender, simply are not aware of the data distributions at remote clients.

Table~\ref{tab:apply_to_non_iid} shows the performance of FLBuff under the above setting. Table~\ref{tab:apply_to_non_iid} shows that FLBuff consistently results at low \texttt{ASR} against different backdoors across various datasets and \NIIDs (see Table~\ref{tab:noniid_bechmark}): most \texttt{ASR} with \FB is low while \texttt{ASR} with other defenses easily exceeds 15\% or even 20\%. When defending against ALIE attack on MNIST, \texttt{ASR} of FLBuff is 0.47\% (IID), 7.31\% (dir), 8.96\% (prob), 10.21\% (qty), 1.30\% (noise), and 6.20\% (qs). Similar \texttt{ASR} can be found for FMNIST, CIFAR10, and IMDB as well, demonstrating its robustness under challenging \NIIDs compared to SOTA defenses. Such results conclude that \FB can handle various \NIIDs well, which most prior defenses cannot. The results also provide evidence for our core intuition in Sect.~\ref{sec:a-unified-view}.


\subsubsection{Ablation Study}
\label{sec:evaluation:ablation}
In this section, we study the impact of each component (the known attacks and known \NIIDs) of \FB on the defense effectiveness. Due to limited space, we defer part of the evaluation results to Appendix~\ref{sec:appenddix-additional-results}.
% \xlnote{For the space limit,we can move the part of knowledge of Non-IIDs,attacks,contributions to the appendix while emphasizing the impact of parameters and the adaptive attack. Other NIIDs result including generated and Federated-MNSIT would be shown here.}



% \textbf{Knowledge of \NIIDs}
% We want to explore how additional knowledge of certain \NIIDs can improve \FB's performance, i.e., Goal 4. Table~\ref{tab:apply_to_non_iid} demonstrates that the performance of FLBuff is markedly affected by the training strategy employed. The three strategies, i.e., iid, iid-dir, and iid-dir-prob, denote that the training set for \FB consists of (1) IID benign data only, (2) IID and dir-based benign data, and (3) IID, dir-based, and prob-based benign data. Such an arrangement serves to demonstrate the impact of additional \NIID knowledge. 

% Table~\ref{tab:apply_to_non_iid} suggests that \FB models trained under purely IID distributions generally exhibit higher \texttt{ASR} when evaluated in \NIID scenarios. For instance, in the BadNet attack on the MNIST dataset, the \texttt{ASR} for the IID strategy is 1.82\% under the IID scenario, but it escalates to 9.73\% for the dir-based scenario and 10.04\% for the prob-based scenario. However, the \texttt{ASR} significantly decreases to 0.43\% and 0.77\%, respectively, when a single \NIID strategy is incorporated during model training. Aside from that such a finding is consistent across various attacks and datasets, we conjecture that the finding is consistent with Proposition~\ref{cor:one-defense-for-all} that the impact of different \NIIDs tend to be `similar'. Hence, a \FB model effective under dir-based \NIID is likely to work under prob-based and/or qty-based \NIID.

% Moreover, models trained with multiple \NIIDs demonstrate superior performance compared to those trained with a single \NIID strategy. For instance, in the DBA attack on the CIFAR10, the \texttt{ASR} for the iid-dir strategy under the prob-based \NIID scenario is 7.20\%, whereas it decreases to 0.90\% for the iid-dir-prob strategy. This indicates that exposure to a broader range of \NIIDs during training enhances the model's generalization ability and its efficacy in defending against attacks in various \NIID settings.



 

% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}[t]{0.23\textwidth}
%         \includegraphics[width=\textwidth]{figures/thr-rate-mpa/mpa_scaling.pdf}
%         \caption{FMNIST, IID, Scaling attack}
%         \label{fig:mpa_scaling}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.23\textwidth}
%         \includegraphics[width=\textwidth]{figures/thr-rate-mpa/mpa_dba.pdf}
%         \caption{FMNIST, IID, DBA attack}
%         \label{fig:mpa_dba}
%     \end{subfigure}
%     \vspace{-5pt}
%     \caption{Applicability of FLBuff to other backdoor attacks.}
%     \label{fig:model_based_mpa}
%     \vspace{-5pt}
% \end{figure}

% \textbf{Knowledge of Attacks.}
% Here, we first explore the setting that \FB is applied for defending against other backdoor attacks that it is not trained for (Goal 3), i.e., we use the labelled samples from the specific attack to train a \FB model and use the trained model for defending against other backdoor attacks. 

% Figure~\ref{fig:model_based_mpa} illustrates the defense performance of \FB when \FB is trained based solely on the BadNet attack (iid-BadNet) and then applied to Scaling and DBA attacks. Due to space limits, we do not include results under other settings such as \FB trained from iid-DBA or iid-Scaling. Our first observation is that FL models without \FB exhibit consistently high \texttt{ASR} across various backdoor attacks, such as Scaling and DBA on the FMNIST dataset. However, with \FB, the \texttt{ASR} significantly decreases across different attacks, demonstrating the effectiveness of \FB from iid-BadNet on attacks like Scaling and DBA. Figure~\ref{fig:model_based_mpa} also includes results when the training set of \FB consists of malicious samples from other attacks, i.e., the training set has diverse attack samples. E.g., BadNet-ALIE means that both BadNet and ALIE samples are used for training. The results suggest that additional attack samples for training improve \FB's performance slightly. %Additionally, models trained to defend against a specific attack type (e.g., BadNet) are also effective in mitigating other attacks (e.g., Scaling, DBA), indicating that \FB's defense mechanisms are broadly applicable and adaptable. 
% Note that all the \texttt{Acc} remains high, confirming that FL models with FLBuff maintain overall great model performance. \texttt{Acc} for other datasets under various \NIIDs can be found in Table~\ref{tab:test_all_benigh} at Appendix~\ref{sec:appenddix-additional-results}.

% %\textbf{Applicability to other backdoor attacks under other Non-IIDs.}
% Table~\ref{tab:apply_to_MPAs_non_iid} consolidate results when \FB trained on a single attack (specifically, on BadNet) is applied to other backdoor attacks. Due to space limits, we do not include results under other settings such as \FB trained from DBA or Scaling. Firstly, we can see that such a \FB model excels in defending against BadNet attack across various datasets and \NIID settings, which is expected as it is trained from BadNet samples. Interestingly, the model further demonstrates moderate effectiveness against other backdoors (i.e., DBA, Scaling, and ALIE), though not at optimal levels. Meanwhile, we found that the \FB model trained with \NIID data generally yields better results than that only using IID data, and incorporating multiple \NIID scenarios further enhances \FB's effectiveness. For instance, the \texttt{ASR} of BadNet drops when adopting one or more \NIIDs compared with only IID.

% \begin{table}[ht]
% \caption{Applicability to other MPAs of FLBuff(IID).}\xl{will change this table into the figures to show partial results}

% \begin{minipage}{0.45\linewidth}
% \centering
% \subcaption{\texttt{ASR}(\%) of Scaling}
% \begin{tabular}{c|cccc}
% \toprule
% \textbf{Dataset}  & \textbf{badnet} & \textbf{badnet-scaling} & \textbf{badnet-dba} & \textbf{badnet-alie} \\
% \midrule
% MNIST & 5.84 & 1.56 & 0.73 & 1.87 \\
% FMNIST & 1.70 & 1.90 & 1.10 & 1.20  \\
% CIFAR10 & 6.20 & 5.30 & 7.10 & 7.60 \\
% IMDB & 5.60 & 4.50 & 4.20 & 4.00  \\
% \bottomrule
% \end{tabular}
% \end{minipage} 

% \vspace{0.2cm}

% \begin{minipage}{0.45\linewidth}
% \centering
% \subcaption{\texttt{ASR}(\%) of DBA}
% \begin{tabular}{c|cccc}
% \toprule
% \textbf{Dataset}  & \textbf{badnet} & \textbf{badnet-scaling} & \textbf{badnet-dba} & \textbf{badnet-alie} \\
% \midrule
% MNIST & 2.19 & 0.84 & 1.04 & 1.25 \\
% FMNIST & 5.80 & 4.50 & 2.30 & 4.90 \\
% CIFAR10 & 8.60 & 3.40 & 3.70 & 6.00 \\
% IMDB & 5.00 & 2.70 & 2.50 & 3.80 \\
% \bottomrule
% \end{tabular}
% \end{minipage} 
% \vspace{0.2cm}

% \begin{minipage}{0.45\linewidth}
% \centering
% \subcaption{\texttt{ASR}(\%) of BadNet}
% \begin{tabular}{c|cccc}
% \toprule
% \textbf{Dataset}  & \textbf{badnet} & \textbf{badnet-scaling} & \textbf{badnet-dba} & \textbf{badnet-alie} \\
% \midrule
% MNIST & 3.81 & 1.77 & 1.73 & 0.34 \\
% FMNIST & 4.52 & 3.69 & 4.22 & 2.05 \\
% CIFAR10 & 5.13 & 3.92 & 4.75 & 3.25 \\
% IMDB & 5.56 & 4.68 & 4.30 & 3.74 \\
% \bottomrule
% \end{tabular}
% \end{minipage} 

% \vspace{0.2cm}

% \begin{minipage}{0.45\linewidth}
% \centering
% \subcaption{\texttt{ASR}(\%) of ALIE}
% \begin{tabular}{c|cccc}
% \toprule
% \textbf{Dataset}  & \textbf{badnet} & \textbf{badnet-scaling} & \textbf{badnet-dba} & \textbf{badnet-alie} \\
% \midrule
% MNIST & 0.42 & 0.35 & 0.31 & 0.21 \\
% FMNIST & 0.63 & 0.49 & 0.36 & 0.17 \\
% CIFAR10 & 3.50 & 4.18 & 3.68 & 3.53 \\
% IMDB & 4.20 & 3.50 & 1.30 & 2.27 \\
% \bottomrule
% \end{tabular}
% \end{minipage} 
% \end{table}








% \textbf{Comparing the contributions from \NIIDs and backdoor attacks.}
% The above results confirm that \FB achieves better performance when \NIID benign and/or additional backdoor samples are used for training. This aligns with Figure~\ref{fig:multi-attack-feasibility} that the displacement of a specific attack and the expansion of a specific \NIID together affect the buffer layer \FB provides. Therefore, we want to figure out which \NIID and which backdoor attack can lead to the maximum improvement. Table~\ref{tab:contribution_mpas_noniids} shows the results of the contributions from different \NIIDs and backdoors to the trained \FB model, emphasizing that the choice of backdoors and/or Non-IIDs for training can impact defense effectiveness. From the table we can see that models trained with DBA and dir-based \NIID demonstrate the most robust defense performance across various backdoors and \NIIDs. It thus suggests that incorporating DBA and dir-based data during training enhances \FB's robustness against attacks more effectively than other combinations. 

% On the contrary, \FB models trained with Scaling and qty-based \NIID exhibit the least effectiveness, indicating that such a combination contributes marginally to \FB.
% Selecting appropriate training conditions, such as combining diverse and challenging MPAs with dir-based Non-IID data, to bolster defense mechanisms in federated learning environments, achieving greater resilience against sophisticated adversarial attacks.

%the contributions from different non-iid
% \begin{table}[ht]
% \fontsize{7}{8}\selectfont
% % \scriptsize
% \centering
% \caption{Contributions from different Non-IIDs and different backdoor attacks to \FB}
% \renewcommand{\arraystretch}{1.2} 
% \label{tab:contribution_mpas_noniids}
% \begin{minipage}{\linewidth}
% \subcaption{Scaling \& DBA}
% \begin{tabular}{c|c|cccc|cccc}
%  \hline
% \multirow{2}{*}{\textbf{iid-}} & \multirow{2}{*}{\textbf{Attack}} & \multicolumn{4}{c|}{\textbf{BadNet}} & \multicolumn{4}{c}{\textbf{DBA}} \\
%  \cline{3-10}
% & & \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty} & \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty} \\
%  \hline
% \multirow{3}{*}{\textbf{-dir}} 
% & BadNet & \textbf{0.39} & 6.45 & 3.50 & \textbf{1.92} & 0.84 & 6.42 & 4.52 & 3.43 \\
% & DBA & 1.50 & \textbf{3.70} & \textbf{3.47} & 2.56 & \textbf{0.25} & \textbf{0.69} & \textbf{1.83} & \textbf{3.10} \\
% & Scaling & 3.53 & 5.05 & 6.78 & 6.20 & 1.45 & 4.52 & 5.80 & 3.35 \\
% & ALIE & 2.66 & 5.59 & 7.24 & 3.60 & 0.61 & 5.42 & 6.71 & 2.52 \\
%  \hline
% \multirow{3}{*}{\textbf{-prob}} 
% & BadNet & 2.00 & 6.80 & 5.30 & 4.84 & 1.67 & 8.20 & 7.54 & 8.29 \\
% & DBA & \textbf{1.60} & \textbf{5.10} & \textbf{4.28} & 4.16 & 0.75 & \textbf{4.45} & \textbf{1.67} & 2.42 \\
% & Scaling & 2.12 & 7.01 & 7.16 & 6.60 & 0.97 & 8.27 & 6.77 & \textbf{1.99} \\
% & ALIE & 2.80 & 8.72 & 4.95 & \textbf{3.52} & \textbf{0.66} & 5.49 & 4.67 & 6.98 \\
%  \hline
% \multirow{3}{*}{\textbf{-qty}} 
% & BadNet & \textbf{0.50} & 5.27 & 3.51 & 2.88 & 1.35 & 6.77 & 5.45 & \textbf{1.01} \\
% & DBA & 0.68 & 5.71 & \textbf{3.09} & 1.73 & 2.69 & 6.47 & \textbf{3.71} & 1.58 \\
% & Scaling & 0.70 & \textbf{3.52} & 3.19 & \textbf{0.79} & \textbf{0.38} & 5.55 & 7.61 & 1.26 \\
% & ALIE & 1.02 & 8.14 & 7.08 & 3.60 & 2.61 & \textbf{5.42} & 4.76 & 2.55 \\
%  \hline
% \end{tabular}
% \end{minipage}

% \vspace{0.3cm}
% \renewcommand{\arraystretch}{1.2} 
% \begin{minipage}{\linewidth}
% \subcaption{BadNet \& ALIE}
% \begin{tabular}{c|c|cccc|cccc}
%  \hline
% \multirow{2}{*}{\textbf{iid-}} & \multirow{2}{*}{\textbf{Attack}} & \multicolumn{4}{c|}{\textbf{Scaling}} & \multicolumn{4}{c}{\textbf{ALIE}} \\
%  \cline{3-10}
% & & \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty} & \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty} \\
%  \hline
% \multirow{3}{*}{\textbf{-dir}} 
% & BadNet & \textbf{0.41} & 7.64 & 6.44 & \textbf{0.10} & 0.80 & 6.18 & 5.84 & 3.67 \\
% & DBA & 0.93 & 1.63 & \textbf{3.53} & 0.31 & 0.50 & 2.61 & \textbf{2.80} & 4.68 \\
% & Scaling & 0.91 & \textbf{0.60} & 3.86 & 5.15 & 2.02 & 6.15 & 7.20 & 5.36 \\
% & ALIE & 1.28 & 6.21 & 8.19 & 5.65 & \textbf{0.27} & \textbf{0.90} & 4.60 & \textbf{1.78} \\
%  \hline
% \multirow{3}{*}{\textbf{-prob}} 
% & BadNet & 1.19 & 8.65 & 7.10 & 8.03 & 1.90 & 6.15 & 4.18 & 6.26 \\
% & DBA & 1.25 & \textbf{3.36} & \textbf{3.34} & \textbf{1.63} & \textbf{0.72} & \textbf{3.45} & 6.93 & \textbf{4.50} \\
% & Scaling & \textbf{0.50} & 6.17 & 5.69 & 6.72 & 1.00 & 5.56 & 4.27 & 5.90 \\
% & ALIE & 1.87 & 9.27 & 10.01 & 5.57 & 1.45 & 5.45 & \textbf{3.53} & 7.50 \\
%  \hline
% \multirow{3}{*}{\textbf{-qty}} 
% & BadNet & 1.69 & 8.35 & 8.60 & 0.90 & 1.01 & \textbf{5.10} & 6.30 & 5.01 \\
% & DBA & \textbf{0.70} & 5.78 & \textbf{3.15} & 1.75 & 2.66 & 6.40 & \textbf{3.65} & 1.54 \\
% & Scaling & 0.71 & \textbf{3.56} & 3.23 & \textbf{0.81} & \textbf{0.36} & 5.49 & 7.55 & \textbf{1.23} \\
% & ALIE & 1.28 & 6.21 & 7.15 & 3.65 & 1.80 & 6.36 & 3.50 & 1.49 \\
%  \hline
% \end{tabular}
% \end{minipage}
% \end{table}


% \begin{table}[ht]
% \centering
% \caption{Contributions from different Non-IIDs and different backdoor attacks to the trained model}
% \label{tab:contribution_mpas_noniids}
% \begin{minipage}{\linewidth}
% \subcaption{Scaling \& DBA}
% \begin{tabular}{c|c|cccc|cccc}
% \toprule
% \multirow{2}{*}{\textbf{iid-}} & \multirow{2}{*}{\textbf{Backdoor attack}} & \multicolumn{4}{c|}{\textbf{BadNet}} & \multicolumn{4}{c}{\textbf{DBA}}  \\
% \cmidrule(lr){3-6} \cmidrule(lr){7-10} 
% & & \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty} & \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty}  \\
% \midrule
% \multirow{3}{*}{\textbf{-dir}} 
% & BadNet & 0.39 & 6.45 & 3.50 & 1.92  & 0.84 & 6.42 & 4.52 & 3.43 \\
% & DBA & 1.50 & 3.70 & 3.47 & 2.56  & 0.25 & 0.69 & 1.83 & 3.10  \\
% & Scaling & 3.53 & 5.05 & 6.78 & 6.20 & 1.45 & 4.52 & 5.80 & 3.35 \\
% & ALIE & 2.66 & 5.59 & 7.24 & 3.60 & 0.61 & 5.42 & 6.71 & 2.52 \\
% \midrule
% \multirow{3}{*}{\textbf{-prob}} 
% & BadNet & 2.00 & 6.80 & 5.30 & 4.84 & 1.67 & 8.20 & 7.54 & 8.29  \\
% & DBA & 1.60 & 5.10 & 4.28 & 4.16 & 0.75 & 4.45 & 1.67 & 2.42 \\
% & Scaling & 2.12 & 7.01 & 7.16 & 6.60 & 0.97 & 8.27 & 6.77 & 1.99  \\
% & ALIE & 2.80 & 8.72 & 4.95 & 3.52 & 0.66 & 5.49 & 4.67 & 6.98 \\
% \midrule
% \multirow{3}{*}{\textbf{-qty}}
% & BadNet & 0.50 & 5.27 & 3.51 & 2.88 & 1.35 &  6.77 & 5.45 & 1.01 \\
% & DBA & 0.68 & 5.71 & 3.09 & 1.73 & 2.69 & 6.47 & 3.71 & 1.58 \\
% & Scaling & 0.70 & 3.52 & 3.19 & 0.79 & 0.38 & 5.55 & 7.61 & 1.26  \\
% & ALIE & 1.02 & 8.14 & 7.08 & 3.60  & 2.61&  5.42 & 4.76 & 2.55 \\
% \bottomrule
% \end{tabular}
% \end{minipage}

% \vspace{0.15cm}

% \begin{minipage}{\linewidth}
% \subcaption{BadNet \& ALIE}
% \begin{tabular}{c|c|cccc|cccc}
% \toprule
% \multirow{2}{*}{\textbf{iid-}} & \multirow{2}{*}{\textbf{Backdoor attack}} & \multicolumn{4}{c|}{\textbf{Scaling}} & \multicolumn{4}{c}{\textbf{ALIE}}  \\
% \cmidrule(lr){3-6} \cmidrule(lr){7-10} 
% & & \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty} & \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty}  \\
% \midrule
% \multirow{3}{*}{\textbf{-dir}} 
% & BadNet & 0.41 & 7.64 & 6.44 & 0.10 & 0.80 & 6.18 & 5.84 & 3.67 \\
% & DBA & 0.93 & 1.63 & 3.53 & 0.31 & 0.50 & 2.61 & 2.80 & 4.68   \\
% & Scaling & 0.91 & 0.60 & 3.86 & 5.15& 2.02 & 6.15 & 7.20 & 5.36 \\
% & ALIE & 1.28 & 6.21 & 8.19 & 5.65 & 0.27 & 0.90 & 4.60 & 1.78\\
% \midrule
% \multirow{3}{*}{\textbf{-prob}}
% & BadNet & 1.19 & 8.65 & 7.10 & 8.03 & 1.90 & 6.15 & 4.18 & 6.26   \\
% & DBA & 1.25 & 3.36 & 3.34 & 1.63  & 0.72 & 3.45 & 6.93 & 4.50  \\
% & Scaling & 0.50 & 6.17 & 5.69 & 6.72 & 1.00 & 5.56 & 4.27 & 5.90  \\
% & ALIE & 1.87 & 9.27 & 10.01 & 5.57& 1.45 & 5.45 & 3.53 & 7.50 \\
% \midrule
% \multirow{3}{*}{\textbf{-qty}} 
% & BadNet & 1.69 & 8.35 & 8.60 & 0.90 & 1.01 &  5.10 & 6.30 & 5.01 \\
% & DBA & 0.70 & 5.78 & 3.15 & 1.75  & 2.66 & 6.40 & 3.65 & 1.54  \\
% & Scaling & 0.71 & 3.56 & 3.23 & 0.81 & 0.36 & 5.49 & 7.55 & 1.23  \\
% & ALIE & 1.28 & 6.21 & 7.15 & 3.65 & 1.80 &  6.36 & 3.50 & 1.49 \\
% \bottomrule
% \end{tabular}
% \end{minipage}
% \end{table}






\subsubsection{Robustness under Different Parameters}
\label{noniid-degree-study}
% In this section, we want to evaluate the robustness of \FB under important hyper-parameters. This is critical because attackers' strategies may vary in terms of malicious ratio and data poisoning rate, while the classification threshold of Sup-CL needs to vary accordingly. Therefore, we decide to discuss the robustness of \FB when facing up with such variances in attack strategies. Due to space limits, we only include results on CIFAR10 and additional results on other datasets such as MNIST, FMNIST and IMDB can be found in Table~\ref{tab:impact_number_client_mnist}, Figure~\ref{fig:noniid-degree-impact-fmnist}, Figure~\ref{fig:noniid-degree-impact-imdb}, Table~\ref{tab:impact_number_client_fmnist}, and Figure~\ref{fig:pdr_dt_impact} in Appendix.
In this section, we evaluate the robustness of \FB under various hyperparameters (i.e., Goal 5). This is critical because attackers' strategies may vary in terms of malicious ratio and data poisoning rate, while the classification threshold of Sup-CL needs to vary accordingly. Due to space limits, we only include results on CIFAR10 and additional results on other datasets can be found in Table~\ref{tab:impact_number_client_mnist}, Table~\ref{tab:impact_number_client_fmnist}, Figure~\ref{fig:noniid-degree-impact-fmnist}, Figure~\ref{fig:noniid-degree-impact-imdb}, and Figure~\ref{fig:pdr_dt_impact} in Appendix.

\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/noniid-degree/noniid_degree_Badnet.pdf}
        \caption{BadNet~\cite{gu2017badnets}}
        \label{fig:noniid_degree_Badnet}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/noniid-degree/noniid_degree_DBA.pdf}
        \caption{DBA~\cite{xie2019dba}}
        \label{fig:noniid_degree_DBA}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/noniid-degree/noniid_degree_Scaling.pdf}
        \caption{Scaling~\cite{bagdasaryan2020backdoor}}
        \label{fig:noniid_degree_Scaling}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/noniid-degree/noniid_degree_ALIE.pdf}
        \caption{ALIE~\cite{baruch2019little}}
        \label{fig:noniid_degree_ALIE}
    \end{subfigure}
    \vspace{-5pt}
    \caption{Impact of the degree of \NIID on FLBuff on CIFAR10. The larger value, the more severe \NIID.}
    \label{fig:noniid-degree-impact}
    \vspace{-5pt}
\end{figure*}
\textbf{Impact of Non-IID degree.}
For easier comparison, we normalize all non-IID degrees on a unified scale ranging from 0.1 to 0.9. Intuitively, a large \NIID degree leads to severe expansion of \NIID from IID, therefore increasing the probability that the resulted benign cluster overlaps with the malicious cluster. See Figure~\ref{fig:small-buffer} for more details. Figure~\ref{fig:noniid-degree-impact} shows the impact of \NIID degree on \FB, from which we have two observations. First, the \texttt{ASR} without \FB increases as the degree of \NIID rises indicating that a larger \NIID degree harms the FL model more severely. Second, when \NIID degree increases, it has only a slight influence on the defense performance of \FB, hence rendering \FB a robust defense towards \NIID degree. {The results for noise and quantity skew can be found in Table~\ref{tab:impact_degree_noise} and Table~\ref{tab:impact_degree_qunt} in Appendix.}


        
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/malicious-rate/rate_attackers_BadNet.pdf}
        \caption{BadNet~\cite{gu2017badnets}}
        \label{fig:rate_attackers_BadNet}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/malicious-rate/rate_attackers_DBA.pdf}
        \caption{DBA~\cite{xie2019dba}}
        \label{fig:rate_attackers_DBA}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/malicious-rate/rate_attackers_Scaling.pdf}
        \caption{Scaling~\cite{bagdasaryan2020backdoor}}
        \label{fig:rate_attackers_Scaling}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{figures/malicious-rate/rate_attackers_ALIE.pdf}
        \caption{ALIE~\cite{baruch2019little}}
        \label{fig:rate_attackers_ALIE}
    \end{subfigure}
    \vspace{-5pt}
    \caption{Impact of the number of malicious clients on FLBuff on CIFAR10.}
    \label{fig:malicious_numbers}
    \vspace{-5pt}
\end{figure*}
\textbf{Impact of the number of malicious clients.}
Intuitively, a larger malicious rate corresponds to a stronger backdoor attack on the chosen FL model. Figure~\ref{fig:malicious_numbers} shows the impact of the number of malicious clients on \FB. First, we observe that malicious models can achieve high \texttt{ASR} without \FB under both IID and \NIID settings, confirming the effectiveness of these backdoors. Secondly, \FB effectively mitigates backdoors, maintaining low \texttt{ASR} values even as the number of malicious clients increases. %, although it starts to decline after surpassing a certain threshold. Despite this drop, \FB remains effective under \NIIDs. 

% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}[b]{0.23\textwidth}
%         \includegraphics[width=\textwidth]{figures/thr-rate-mpa/pdr_result.pdf}
%         \caption{Impact of data poisoning rate}
%         \label{fig:data_poisoning_rate}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.23\textwidth}
%         \includegraphics[width=\textwidth]{figures/thr-rate-mpa/detection_thr.pdf}
%         \caption{Impact of classification threshold}
%         \label{fig:detection_threshold}
%     \end{subfigure}
%     \vspace{-5pt}
%     \caption{Impact of data poisoning rate and classification threshold. Dataset: FMNIST; \NIID: dir-0.3; Attack: Scaling~\cite{bagdasaryan2020backdoor}.}
%     \label{fig:pdr_dt_impact}
%     \vspace{-5pt}
% \end{figure}

\textbf{Impact of data poisoning rate.} 
Similarly, a larger data poisoning rate corresponds to a stronger backdoor attack on the chosen FL model. Figure~\ref{fig:data_poisoning_rate} showcases the effect of varying data poisoning rates on \FB. We can see that as the poisoning rate increases, the \texttt{ASR} without defense increases as well as each malicious model update becomes more effective on the targeted FL model. The increasing  rate, however, has only a slight impact on \FB, which results in low \texttt{ASR}s even under severe poisoning.

\textbf{Impact of classification threshold $\gamma$.} 
Figure~\ref{fig:detection_threshold} illustrates the impact of classification thresholds on \FB. When the threshold is set too low at 0.2, \FB experiences a slight influence, while setting the classification threshold too high at 0.9 slightly affects the main accuracy. It is crucial to set a reasonable threshold to ensure the inclusion of benign participants while maintaining strong defense.
% \textbf{Model poisoning rate}. Here we want to see.
%  \xl{how to set Model poisoning rate?}


% \begin{table}[t]
% \fontsize{10}{10}\selectfont
% \centering
% \renewcommand{\arraystretch}{1.2} 
% \caption{FLBuff under adaptive attacks}
% \label{tab:adaptive_attack_table}
% \begin{minipage}{0.95\columnwidth}
% \centering
% \subcaption{BadNet \& DBA. Same \NIIDs as Sect.~\ref{non-iid-datasets}}
% \resizebox{0.95\columnwidth}{!}{
% \begin{tabular}{c|cccccc|cccccc}
% \hline
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{6}{c|}{\textbf{BadNet}} & \multicolumn{6}{c}{\textbf{DBA}}  \\
% \cline{2-13}
% &  \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty} & \textbf{noise} & \textbf{qs} & \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty} & \textbf{noise} & \textbf{qs}  \\
% \hline
% MNIST   & \textbf{0.12} & 0.31 & 1.01 & 0.56 & 0.93 & 1.04 & 0.86 & \textbf{0.73} & 1.57 & 0.58 & 0.94 & 1.26\\
% FMNIST  & 1.03 & 0.95 & \textbf{0.76} & 0.73 & 1.00 & 1.25 & 0.65 & \textbf{0.35} & 0.83 & 0.42 & 0.77 & 1.15 \\
% CIFAR10 & 0.63 & 1.11 & 1.53 & \textbf{0.56} & 1.20 & 1.41 & 1.03 & 2.22 & 1.75 & 0.94 & \textbf{0.92} & 1.70 \\
% IMDB    & 1.15 & 1.39 & 2.25 & \textbf{0.88} & 0.86 & 1.10 & \textbf{0.45} & 1.09 & 0.51 & 0.83 & 0.60 & 1.32 \\
% \hline
%  \end{tabular}
% }
% \end{minipage}

% \vspace{0.3cm}

% \begin{minipage}{0.95\columnwidth}
% \centering
% \subcaption{Scaling \& ALIE. Same \NIIDs as Sect. ~\ref{non-iid-datasets}}
% \resizebox{0.95\columnwidth}{!}{
% \begin{tabular}{c|cccccc|cccccc}
% \hline
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{6}{c|}{\textbf{Scaling}} & \multicolumn{6}{c}{\textbf{ALIE}}  \\
% \cline{2-13}
% &  \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty} & \textbf{noise} & \textbf{qs} & \textbf{iid} & \textbf{dir} & \textbf{prob} & \textbf{qty} & \textbf{noise} & \textbf{qs}  \\
% \hline
% MNIST    & \textbf{0.20} & 0.42 & 1.37 & 0.35 & 0.72 & 0.93 & 0.40 & \textbf{0.37} & 1.11 & 0.45 & 0.52 & 1.27\\
% FMNIST   & 0.96 & 1.35 & 1.86 & \textbf{0.60} & 1.38 & 1.50 & 0.55 & 1.04 & 1.27 & \textbf{0.10} & 0.72 & 1.40 \\
% CIFAR10  & 1.15 & 1.50 & 1.09 & \textbf{1.06} & 0.73 & 1.09 & 0.83 & 0.60 & 0.96 & \textbf{0.12} & 0.98 & 1.10 \\
% IMDB     & 0.57 & 1.38 & 1.03 & \textbf{0.42} & 1.00 & 1.34 & 0.79 & 0.87 & 1.03 & \textbf{0.65} & 0.92 & 1.18\\
% \hline
% \end{tabular}
% }
% \end{minipage}
% \end{table}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/adaptive-attack/adaptive_mnist.pdf}
        \caption{MNIST. Non-IID degree: 0.3}
        \label{fig:adaptive_mnist}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/adaptive-attack/adaptive_fmnist.pdf}
        \caption{FMNIST. Non-IID degree: 0.3}
        \label{fig:adaptive_fmnist}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/adaptive-attack/adaptive_cifar.pdf}
        \caption{CIFAR10. Non-IID degree: 0.3}
        \label{fig:adaptive_cifar}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/adaptive-attack/adaptive_imdb.pdf}
        \caption{IMDB. Non-IID degree: 0.3}
        \label{fig:adaptive_imdb}
    \end{subfigure}
    \vspace{-5pt}
    \caption{Performance of FLBuff against adaptive attacks.}
    \label{fig:flbuff_adaptive_performance}
    \vspace{-5pt}
\end{figure}


% \xl{more adaptive strategy-->method/optimization/normalization-->result analysis}
\subsubsection{Resilience to Adaptive Attacks under \NIIDs} 
As in prior defenses, we expect that resilience to adaptive attacks is critical for a defense (i.e., Goal 5). When it comes to backdoors, given knowledge about \FB, a backdoor attacker's goal is to use adaptive attacks for bypassing \FB while successfully attacking the victim FL model. 

The key differences of our evaluations of adaptive attacks from other works are (1) prior works seldom evaluated defense performance against adaptive attacks under \NIIDs while we include five \NIIDs. In fact, \NIID settings are necessary for evaluating defenses against adaptive attacks because \NIIDs effectively facilitate adaptive attacks, i.e., reducing distinguishability between benign and malicious updates. (2) As shown below, we normalize the loss terms in the formulation of adaptive attacks to make sure that the formulation indeed generates optimal malicious updates.

The strategy of the adaptive attacker we consider is to craft her malicious model updates and the corresponding PLRs so that they resemble those of benign model updates. As a result, the formulation of such an adaptive attack is to minimize a combination of loss from (1) targeted backdoored inputs and clean data, (2) the distance between a crafted malicious update and average benign ones, and (3) the distance between the PLR of a crafted malicious update and that of average benign model updates. In the end, we formulate the adaptive attack as follows: 

% \begin{equation}
%     \begin{aligned}
%         \arg\min_{\delta_{mal}} \quad L(\mathcal{D}_{mal}) + \lambda L(\mathcal{D}_{train}) + \rho \lVert \delta_{mal}-\bar{\delta}_{ben}\rVert\\ + \eta d_{plr}.
%     \end{aligned}
%     \label{eq:adaptive}
% \end{equation}

\begin{equation}
    \begin{aligned}
        \arg\min_{\delta_{mal}} \quad L(\mathcal{D}_{mal}) + \lambda L(\mathcal{D}_{train}) + \rho \Tilde{\Delta d_{\delta}} + \eta \Tilde{d_{plr}},
    \end{aligned}
    \label{eq:adaptive-attack}
\end{equation}

% \begin{equation}
% \label{equ:adaptive-loss}
%     \text{arg min}_{\delta_{\text{mal}}} L(D_{\text{mal}}) + \lambda L(D_{\text{clean}}) + \rho \|\delta_{\text{mal}} - \bar{\delta}_{\text{ben}}\| + \eta d_{\text{plr}}
% \end{equation}

% \xlnote{ours:loss = loss-class+ rho-reg * normalized-loss-reg * max-loss-class + rho-plr * normalized-d-plr * max-loss-class}
\noindent where $L(\mathcal{D}_{mal})$ denotes the loss on targeted backdoored inputs, $L(\mathcal{D}_{train})$ the loss on clean dataset, $\Tilde{\Delta d_{\delta}} = \frac{\lVert \delta_{mal}-\bar{\delta}_{ben}\rVert}{\lVert \delta_{mal}-\bar{\delta}_{ben}\rVert_{max}}$ the normalized distance between malicious model updates and average benign ones, and finally \(\Tilde{d_{plr}}=\frac{d_{plr}}{d_{plr,max}}\) the normalized distance between the PLRs of malicious model updates and the average one of benign models. $\lambda$, $\rho$, and $\eta$ are the corresponding coefficients for different loss terms we obtain from the Algorithm~\ref{alg:greedy-search}. 
 % This formula aims to mislead the global model into outputting target labels for selected inputs while concealing its malicious intent. \xlnote{Should be noted? -- We utilized a greedy search method to determine the appropriate hyperparameters in equation~\ref{equ:adaptive-loss}. More details are provided in the Appendix.}Appendix~\ref{appendxi:greedy-search}.

We use two types of \texttt{ASR} to evaluate the performance of \FB against adaptive attacks: the one when the attacker's malicious updates are aggregated as benign ones into the global model and the one aggregated by \FB. Obviously, the larger differences between the two, the more resilient \FB is towards adaptive attacks. 
Table~\ref{tab:adaptive_attack_table} lists the resulted ASRs of the above adaptive attack on \FB. The results confirms that \FB still works well against adaptive attacks particularly across various datasets and all the five \NIIDs. Figure~\ref{fig:flbuff_adaptive_performance} further shows that the adaptive attack can achieve a high \texttt{ASR} without \FB, meaning that such an attack can succeed in attacking the victim FL model. When \FB is deployed as the defense, the performance of the adaptive attack drops significantly. Such results confirm that it is challenging for adaptive attacks to bypass FLBuff and simultaneously achieve their malicious objectives. Similar results are shown in Figure~\ref{fig:adaptriv_appenix} at Appendix~\ref{sec:appendix-adaptive} for 0.5 \NIID degree.





